FastGRN: Few-Step Generative Refinement Networks

Generative Refinement Networks (GRN) generate an image by repeatedly re-predicting and refining every token of a discrete latent. They reach high fidelity, but need dozens of Markov steps. We therefore train few-step GRNs on the distribution of their own samples. We use its own uniform-state corruption to perform distribution matching on discrete tokens, which lets a discrete generator learn by backpropagation, and we pair noise with samples in the manner of rectified flow. We find that the steps of a few-step GRN do not carry the same amount of information or the same repair load. We therefore exploit its discrete refinement during training and build few-step GRNs in three parts. Oversampling samples the student with more steps than it was trained for and refines its judge on these samples. Non-uniform sampling trains only the last step and hands it most of the information at sampling time. Refinement confidence keeping holds on to the tokens the student is already sure of. We train a fast class-conditional generator on ImageNet 256 and, with the same method, a 2B text-to-image model. On ImageNet 256, the 3-step FastGRN beats the FID of GRN. On a 2B binary-token text-to-image GRN, a 4-step student also nearly matches the GenEval of GRN-T2I 2B.

==> tables/tab_ablation_c2i.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Ablations on ImageNet $256^2$ (GRN-B).} (a): 2-step students, FID-10k at 10k iterations; (b): FID-50k. Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:abl_c2i}
\footnotesize
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{@{}lrrrrl@{}}
\toprule
Setting & FID$\downarrow$ & Best (it.) & Prec. & Rec. & Training \\
\midrule
\grpline{6}{(a) Initialization $\times$ objective}
Fine-tuned init. without window & 358.3 & 17.69 (8k) & 0.001 & 0.045 & collapse 7.9k \\
Paired-noise init. without window & 332.8 & 7.87 (4k) & 0.020 & 0.442 & collapse 6.4k \\
Fine-tuned init. with window & 9.85 & 9.85 (10k) & 0.632 & 0.758 & stable \\
Paired-noise init. with window & \textbf{6.65} & 6.59 (6k) & 0.692 & 0.783 & stable \\
\midrule
\grpline{6}{(b) Objective variants (FID-50k)}
No window (4 steps) & 4.63 & \multicolumn{3}{l}{(FID-10k 6.97)} & stable \\
Window (4 steps) & 3.99 & \multicolumn{3}{l}{(FID-10k 6.42)} & stable \\
Window (2 steps) & 4.17 & \multicolumn{3}{l}{(FID-10k 6.65)} & stable \\
single $q{=}0.4$ (2 steps) & 4.15 & \multicolumn{3}{l}{(FID-10k 6.56)} & stable \\
No window + anchor $\lambda{=}10^{-3}$ & \na & \multicolumn{3}{c}{\na} & collapse 3.4k \\
No window + anchor $\lambda{=}5{\cdot}10^{-4}$ & \na & \multicolumn{3}{c}{\na} & collapse 4.2k \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/tab_ablation_t2i.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Ablations on text-to-image (GRN-T2I, $256^2$, LoRA students).} All rows: 2 sampling steps, paired-noise init., fine-tuned real score unless varied. Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:abl_t2i}
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\begin{tabular}{@{}lrrrrl@{}}
\toprule
Setting & GenEval$\uparrow$ & FID-T$\downarrow$ & HPS$\uparrow$ & Div.$\uparrow$ & Healthy \\
\midrule
\grpline{6}{(a) Initialization at $q_{\max}{=}0.4$ (1k it.)}
Fine-tuned init. & \na & 48.6 & 25.51 & 0.73 & no \\
Paired-noise init. & \na & \textbf{42.1} & \textbf{26.16} & \textbf{0.90} & yes \\
\midrule
\grpline{6}{(b) Real score at $q_{\max}{=}0.4$ (2k it.)}
Guided teacher & 0.602 & 49.9 & 26.11 & 0.85 & yes \\
Fine-tuned & \textbf{0.637} & \textbf{41.0} & \textbf{26.38} & \textbf{0.90} & yes \\
\midrule
\grpline{6}{(c) Window $q_{\max}$ (2k it.\ unless noted)}
$0.40$ & 0.637 & 41.0 & 26.38 & 0.90 & yes \\
$0.55$ & 0.661\,{\scriptsize(+0.025)} & 39.1 & 26.58 & 0.91 & yes \\
$0.95$ (no window)$^\ast$ & 0.661\,{\scriptsize(+0.024)} & 37.6 & 26.71 & 0.90 & yes \\
$0.95$ (no window)$^\dagger$ & 0.678\,{\scriptsize(+0.041)} & 37.4 & 26.66 & 0.91 & yes$^v$ \\
\quad same with 8k it. & 0.676\,{\scriptsize(+0.024)$^w$} & 38.4 & 26.87 & 0.91 & no$^v$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_c2i_fewstep.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Few-step sampling without distribution matching fails.} FID-10k on ImageNet $256^2$ versus the number of sampling steps. Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:fewstep}
\footnotesize
\setlength{\tabcolsep}{3.4pt}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Sampling steps $N$ & 2 & 4 & 8 & 16 \\
\midrule
\grpline{5}{GRN-B (teacher at 79 NFE: 6.24)}
GRN-B with fewer steps$^n$ & 112.5 & 49.6 & 10.9 & \na \\
Fine-tuned GRN & 156.9 & 68.3 & 16.7 & 9.56 \\
Paired-noise GRN & 60.8 & 26.9 & 13.0 & 8.68 \\
Matching without window \comp{best before collapse} & 7.87$^c$ & 6.97 & \na & \na \\
\regrn{} (\tagW) & 6.65 & 6.42 & \na & \na \\
\midrule
\grpline{5}{GRN-L}
GRN-L with fewer steps$^n$ & 147.8 & 84.1 & 23.6 & \na \\
Fine-tuned GRN & 163.7 & 89.9 & 22.7 & \na \\
Paired-noise GRN & 82.8 & 39.3 & 15.8 & \na \\
\regrn{} (\tagW) & 6.07 & 5.42 & \na & \na \\
\regrn{} (\tagW+\tagEH)$^h$ & 5.51 & \na & \na & \na \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_c2i_full.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Class-conditional ImageNet $256^2$, all rows and columns} (Tab.~\ref{tab:c2i} shows a subset). FID and IS on 50k samples. $\times$T.: FID relative to the method's own teacher; P$_\mathrm{T}$\,/\,R$_\mathrm{T}$: precision\,/\,recall against 50k teacher samples; ms: batch-1 latency on an RTX 4090, decoding included. Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:c2i_full}
\footnotesize
\setlength{\tabcolsep}{1.6pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Method & Steps & NFE & FID$\downarrow$ & $\times$T.$\downarrow$ & IS$\uparrow$ & P$_\mathrm{T}$ & R$_\mathrm{T}$ & ms$\downarrow$ \\
\midrule
\grpline{9}{GRN-B (130M)}
Teacher & 50 & 79 & 3.73 & \na & 305.9 & 0.733 & 0.730 & 835 \\
GRN-B & 16 & 25 & 3.37 & 0.90 & 287.2 & 0.690 & 0.719 & \na \\
GRN-B & 14 & 22 & 3.51 & 0.94 & 282.5 & 0.681 & 0.720 & \na \\
GRN-B & 12 & 19 & 3.60 & 0.96 & 278.0 & 0.668 & 0.702 & \na \\
GRN-B & 10 & 15 & 4.74 & 1.27 & 228.5 & 0.593 & 0.711 & \na \\
GRN-B & 8 & 12 & 8.13 & 2.18 & 189.8 & 0.540 & 0.687 & \na \\
Fine-tuned GRN & 8 & 8 & 14.0 & 3.76 & 151.0 & 0.547 & 0.704 & \na \\
Paired-noise GRN & 4 & 4 & 24.1 & 6.47 & 114.9 & 0.472 & 0.702 & 94 \\
Paired-noise GRN & 2 & 2 & 58.2 & 15.60 & 47.2 & 0.349 & 0.662 & 66 \\
Matching without window & 2 & 2 & 5.39 & 1.45 & 244.4 & 0.670 & 0.706 & 66 \\
\cmidrule{1-9}
\regrn{} \comp{\tagW+\tagRS} & 4 & 4 & 3.95 & 1.06 & 310.5 & 0.735 & 0.698 & 94 \\
\regrn{} \comp{\tagW+\tagRS+\tagSB} & 4 & 4 & 4.02 & 1.08 & 301.3 & 0.730 & 0.701 & 94 \\
\regrn{} \comp{\tagW} & 4 & 4 & 3.99 & 1.07 & 277.4 & 0.702 & 0.726 & 94 \\
\regrn{} \comp{\tagW+\tagSB+\tagEH} & 2 & 2 & 3.73 & 1.00 & 298.6 & 0.690 & 0.719 & 66 \\
\regrn{} \comp{\tagW+\tagSB} & 2 & 2 & 3.83 & 1.03 & 306.8 & 0.713 & 0.707 & 66 \\
\regrn{} \comp{\tagW} & 2 & 2 & 4.17 & 1.12 & 277.6 & 0.687 & 0.722 & 66 \\
\regrn{} \comp{\tagW+\tagSB+\tagEH} & 4 & 4 & \textbf{3.42} & 0.92 & 317.3 & 0.683 & 0.671 & 94 \\
\regrn{} \comp{\tagW+\tagSB+\tagEH} & 3 & 3 & 3.42 & 0.92 & 318.8 & 0.704 & 0.689 & \na \\
\midrule
\grpline{9}{GRN-L (458M)}
Teacher & 50 & 79 & 2.65 & \na & 319.8 & 0.728 & 0.729 & 1292 \\
\regrn{} \comp{\tagW} & 4 & 4 & 3.03 & 1.15 & 302.7 & 0.734 & 0.697 & 111 \\
\regrn{} \comp{\tagW+\tagEH+\tagCK} & 2 & 2 & 3.03 & 1.15 & 297.7 & 0.714 & 0.716 & 75 \\
\regrn{} \comp{\tagW+\tagEH} & 2 & 2 & 3.09 & 1.17 & 296.4 & 0.716 & 0.710 & 75 \\
\regrn{} \comp{\tagW+\tagEH+\tagCK+\tagSB} & 2 & 2 & 2.85 & 1.08 & 313.9 & 0.724 & 0.706 & 75 \\
\regrn{} \comp{\tagW+\tagEH+\tagCK} & 3 & 3 & \textbf{2.57} & 0.97 & 316.4 & 0.723 & 0.703 & \na \\
\regrn{} \comp{\tagW+\tagEH+\tagCK} & 3 & 3 & 2.70 & 1.02 & 316.6 & 0.733 & 0.694 & \na \\
\regrn{} \comp{\tagW+\tagEH+\tagCK} & 3 & 3 & 2.94 & 1.11 & 329.9 & 0.747 & 0.685 & \na \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/tab_c2i_main.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Class-conditional ImageNet $256^2$.} ms: time per image on one RTX 4090; FID and IS on 50k samples; $\times$T.: FID relative to the teacher. More rows: Tab.~\ref{tab:c2i_full}. Notes: Sec.~\ref{sec:supp_tabnotes}.}
\label{tab:c2i}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
Method & Steps & NFE & ms$\downarrow$ & FID$\downarrow$ & $\times$T.$\downarrow$ & IS$\uparrow$ \\
\midrule
\grpline{7}{GRN-B (130M)}
Teacher & 50 & 79 & 835 & 3.73 & \na & 305.9 \\
GRN-B & 8 & 12 & \na & 8.13 & 2.18 & 189.8 \\
Fine-tuned GRN & 8 & 8 & \na & 14.0 & 3.76 & 151.0 \\
Paired-noise GRN & 2 & 2 & 66 & 58.2 & 15.60 & 47.2 \\
Matching without window & 2 & 2 & 66 & 5.39 & 1.45 & 244.4 \\
\cmidrule{1-7}
\regrn{} \comp{\tagW+\tagRS} & 4 & 4 & 94 & 3.95 & 1.06 & 310.5 \\
\regrn{} \comp{\tagW} & 2 & 2 & 66 & 4.17 & 1.12 & 277.6 \\
\regrn{} \comp{\tagW+\tagSB} & 2 & 2 & 66 & 3.83 & 1.03 & 306.8 \\
\regrn{} \comp{\tagW+\tagSB+\tagEH} & 2 & 2 & 66 & 3.73 & 1.00 & 298.6 \\
\regrn{} \comp{\tagW+\tagSB+\tagEH} & 3 & 3 & \na & \textbf{3.42} & 0.92 & 318.8 \\
\midrule
\grpline{7}{GRN-L (458M)}
Teacher & 50 & 79 & 1292 & 2.65 & \na & 319.8 \\
\regrn{} \comp{\tagW} & 4 & 4 & 111 & 3.03 & 1.15 & 302.7 \\
\regrn{} \comp{\tagW+\tagEH} & 2 & 2 & 75 & 3.09 & 1.17 & 296.4 \\
\regrn{} \comp{\tagW+\tagEH+\tagCK} & 2 & 2 & 75 & 3.03 & 1.15 & 297.7 \\
\regrn{} \comp{\tagW+\tagEH+\tagCK+\tagSB} & 2 & 2 & 75 & 2.85 & 1.08 & 313.9 \\
\regrn{} \comp{\tagW+\tagEH+\tagCK} & 3 & 3 & \na & \textbf{2.57} & 0.97 & 316.4 \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/tab_compare.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Few-step students of discrete generators on ImageNet $256^2$}, as reported. Params in millions; $\times$T.: FID relative to the method's own teacher. Notes: Sec.~\ref{sec:supp_tabnotes}.}
\label{tab:compare}
\footnotesize
\setlength{\tabcolsep}{3pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llrrrr@{}}
\toprule
Method & Teacher & Params & NFE & FID$\downarrow$ & $\times$T.$\downarrow$ \\
\midrule
\ctx{Di[M]O~\cite{zhu2025dimo}} & \ctx{MaskGIT} & \ctx{174} & \ctx{1} & \ctx{6.91} & \ctx{1.05} \\
\ctx{FPD~\cite{wang2026fpd}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{1} & \ctx{6.90} & \ctx{1.05} \\
\ctx{Soft-Di[M]O$^g$~\cite{zhu2026softdimo}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{1} & \ctx{6.40} & \ctx{0.97} \\
\ctx{Di[M]O~\cite{zhu2025dimo}\cite{zhu2026softdimo}} & \ctx{MaskBit} & \ctx{305} & \ctx{1} & \ctx{2.89} & \ctx{1.74} \\
\ctx{Soft-Di[M]O$^g$~\cite{zhu2026softdimo}} & \ctx{MaskBit} & \ctx{305} & \ctx{1} & \ctx{1.96} & \ctx{1.18} \\
\ctx{Soft-Di[M]O$^g$~\cite{zhu2026softdimo} (longer)} & \ctx{MaskBit} & \ctx{305} & \ctx{1} & \ctx{1.56} & \ctx{0.94} \\
\ctx{DD2~\cite{liu2025dd2}} & \ctx{VAR-d20} & \ctx{619} & \ctx{1} & \ctx{5.43} & \ctx{1.60} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{VAR-d16} & \ctx{327} & \ctx{2} & \ctx{7.82} & \ctx{1.87} \\
\ctx{SDTT~\cite{deschenaux2025sdtt}\cite{redi2025}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{4$^c$} & \ctx{8.97} & \ctx{\na} \\
\ctx{ReDi~\cite{redi2025}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{4$^c$} & \ctx{7.58} & \ctx{\na} \\
\ctx{Di4C-d~\cite{hayakawa2025di4c}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{4$^c$} & \ctx{6.57} & \ctx{1.00} \\
\ctx{DAG~\cite{ouyang2026dag}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{4} & \ctx{7.81} & \ctx{\na} \\
\midrule
\regrn{}-B & GRN-B & 130 & 2 & 3.73 & 1.00 \\
\regrn{}-L & GRN-L & 458 & 2 & 2.85 & 1.08 \\
\regrn{}-L & GRN-L & 458 & 3 & 2.57 & \textbf{0.97} \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/tab_compare_ctx.tex <==
\begin{table}[t]
\centering
\caption{\textbf{More few-step generators on ImageNet $256^2$}, as reported by each paper ($\times$T.\ as in Tab.~\ref{tab:compare}; parameters in millions). Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:compare_ctx}
\footnotesize
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Method & Base & Params & NFE & FID$\downarrow$ & $\times$T.$\downarrow$ & IS$\uparrow$ \\
\midrule
\grpline{7}{Further discrete students}
\ctx{SDTT~\cite{deschenaux2025sdtt}\cite{redi2025}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{1$^c$} & \ctx{90.40} & \ctx{\na} & \ctx{14} \\
\ctx{ReDi~\cite{redi2025}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{1$^c$} & \ctx{37.43} & \ctx{\na} & \ctx{49} \\
\ctx{ReDi~\cite{redi2025} (2 rounds)} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{1$^c$} & \ctx{21.80} & \ctx{\na} & \ctx{90} \\
\ctx{ReDi~\cite{redi2025} (2 rounds)} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{4$^c$} & \ctx{7.86} & \ctx{\na} & \ctx{240} \\
\ctx{ReDi-distill~\cite{redi2025}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{1$^c$} & \ctx{11.68} & \ctx{\na} & \ctx{182} \\
\ctx{Di4C~\cite{hayakawa2025di4c}} & \ctx{MaskGIT} & \ctx{174\rlap{$^\dagger$}} & \ctx{4$^c$} & \ctx{6.79} & \ctx{1.03} & \ctx{209.2} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{VAR-d16} & \ctx{327} & \ctx{1} & \ctx{9.94} & \ctx{2.37} & \ctx{193.6} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{VAR-d20} & \ctx{635} & \ctx{1} & \ctx{9.55} & \ctx{2.85} & \ctx{197.2} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{VAR-d20} & \ctx{635} & \ctx{2} & \ctx{7.33} & \ctx{2.19} & \ctx{204.5} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{VAR-d24} & \ctx{1090} & \ctx{1} & \ctx{8.92} & \ctx{3.55} & \ctx{202.8} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{VAR-d24} & \ctx{1090} & \ctx{2} & \ctx{6.95} & \ctx{2.77} & \ctx{222.5} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{LlamaGen-B} & \ctx{98.3} & \ctx{1} & \ctx{15.50} & \ctx{2.86} & \ctx{135.4} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{LlamaGen-B} & \ctx{98.3} & \ctx{2} & \ctx{11.17} & \ctx{2.06} & \ctx{154.8} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{LlamaGen-L} & \ctx{326} & \ctx{1} & \ctx{11.35} & \ctx{2.76} & \ctx{193.6} \\
\ctx{DD1~\cite{liu2025distilleddecoding}} & \ctx{LlamaGen-L} & \ctx{326} & \ctx{2} & \ctx{7.58} & \ctx{1.84} & \ctx{237.5} \\
\ctx{DD2~\cite{liu2025dd2}} & \ctx{VAR-d16} & \ctx{329} & \ctx{1} & \ctx{6.21} & \ctx{1.50} & \ctx{213.0} \\
\ctx{DD2~\cite{liu2025dd2}} & \ctx{VAR-d24} & \ctx{1040} & \ctx{1} & \ctx{5.06} & \ctx{1.77} & \ctx{254.7} \\
\ctx{DD2~\cite{liu2025dd2} (longer)} & \ctx{VAR-d24} & \ctx{1040} & \ctx{1} & \ctx{4.91} & \ctx{1.72} & \ctx{282.2} \\
\ctx{DD2~\cite{liu2025dd2}} & \ctx{LlamaGen-L} & \ctx{335} & \ctx{1} & \ctx{8.59} & \ctx{2.09} & \ctx{229.1} \\
\ctx{DD2~\cite{liu2025dd2} (longer)} & \ctx{LlamaGen-L} & \ctx{335} & \ctx{1} & \ctx{7.58} & \ctx{1.84} & \ctx{238.7} \\
\midrule
\grpline{7}{Native discrete samplers}
\ctx{MaskGIT-PyTorch~\cite{besnier2023maskgitpytorch}} & \ctx{\na} & \ctx{174} & \ctx{2$^c$} & \ctx{91.35} & \ctx{\na} & \ctx{13.4} \\
\ctx{MaskGIT-PyTorch~\cite{besnier2023maskgitpytorch}} & \ctx{\na} & \ctx{174} & \ctx{4$^c$} & \ctx{10.73} & \ctx{\na} & \ctx{192.3} \\
\ctx{MaskGIT-PyTorch~\cite{besnier2023maskgitpytorch}} & \ctx{\na} & \ctx{174} & \ctx{8$^c$} & \ctx{6.66} & \ctx{\na} & \ctx{221.6} \\
\ctx{MaskGIT-PyTorch~\cite{besnier2023maskgitpytorch}} & \ctx{\na} & \ctx{174} & \ctx{16$^c$} & \ctx{6.60} & \ctx{\na} & \ctx{224.1} \\
\ctx{MaskGIT~\cite{chang2022maskgit}} & \ctx{\na} & \ctx{227} & \ctx{8} & \ctx{6.18} & \ctx{\na} & \ctx{182.1} \\
\ctx{Token-Critic~\cite{lezama2022tokencritic}} & \ctx{\na} & \ctx{\na} & \ctx{36} & \ctx{4.69} & \ctx{\na} & \ctx{174.5} \\
\ctx{AutoNAT-S~\cite{ni2024autonat}} & \ctx{\na} & \ctx{46} & \ctx{4$^c$} & \ctx{4.30} & \ctx{\na} & \ctx{249.7} \\
\ctx{AdaNAT-S~\cite{ni2024adanat}} & \ctx{\na} & \ctx{58} & \ctx{4$^c$} & \ctx{4.54} & \ctx{\na} & \ctx{\na} \\
\ctx{MaskGIL-B~\cite{xin2025maskgil}} & \ctx{\na} & \ctx{111} & \ctx{8$^c$} & \ctx{5.64} & \ctx{\na} & \ctx{230.0} \\
\ctx{MaskGIL-L~\cite{xin2025maskgil}} & \ctx{\na} & \ctx{343} & \ctx{8$^c$} & \ctx{4.01} & \ctx{\na} & \ctx{281.1} \\
\ctx{ReMDM~\cite{wang2025remdm}} & \ctx{MaskGIT} & \ctx{\na} & \ctx{16} & \ctx{7.40} & \ctx{\na} & \ctx{145.3} \\
\ctx{DDPD~\cite{liu2025ddpd}} & \ctx{TiTok-S-128} & \ctx{574} & \ctx{16} & \ctx{5.71} & \ctx{\na} & \ctx{201.7} \\
\ctx{Informed corr.~\cite{zhao2024informed}} & \ctx{MD4} & \ctx{400} & \ctx{17} & \ctx{5.78} & \ctx{\na} & \ctx{212.5} \\
\ctx{ReCAP~\cite{liu2025recap}} & \ctx{MaskGIT-r} & \ctx{194} & \ctx{16} & \ctx{5.02} & \ctx{\na} & \ctx{166.6} \\
\ctx{TiTok-B-64~\cite{yu2024titok}} & \ctx{\na} & \ctx{177} & \ctx{8} & \ctx{3.08} & \ctx{\na} & \ctx{192.5} \\
\ctx{VAR-d16~\cite{tian2024var} ($-$2 scales)} & \ctx{\na} & \ctx{310} & \ctx{8} & \ctx{40.09} & \ctx{\na} & \ctx{56.8} \\
\ctx{VAR-d16~\cite{tian2024var} ($-$1 scale)} & \ctx{\na} & \ctx{310} & \ctx{9} & \ctx{9.52} & \ctx{\na} & \ctx{178.9} \\
\midrule
\grpline{7}{Continuous latents}
\ctx{MeanFlow-B/2~\cite{geng2025meanflow}} & \ctx{\na} & \ctx{131} & \ctx{1} & \ctx{6.17} & \ctx{\na} & \ctx{\na} \\
\ctx{MeanFlow-L/2~\cite{geng2025meanflow}} & \ctx{\na} & \ctx{459} & \ctx{1} & \ctx{3.84} & \ctx{\na} & \ctx{\na} \\
\ctx{$\alpha$-Flow-B/2~\cite{zhang2026alphaflow}} & \ctx{\na} & \ctx{131} & \ctx{2} & \ctx{5.01} & \ctx{\na} & \ctx{\na} \\
\ctx{iMF-B/2~\cite{geng2026imf}} & \ctx{\na} & \ctx{89} & \ctx{1} & \ctx{3.39} & \ctx{\na} & \ctx{255.3} \\
\ctx{iMF-L/2~\cite{geng2026imf}} & \ctx{\na} & \ctx{409} & \ctx{1} & \ctx{1.86} & \ctx{\na} & \ctx{276.6} \\
\ctx{Drifting-L/2~\cite{deng2026drifting}} & \ctx{\na} & \ctx{463} & \ctx{1} & \ctx{1.54} & \ctx{\na} & \ctx{258.9} \\
\ctx{FreeFlow-XL/2~\cite{tong2026freeflow}} & \ctx{\na} & \ctx{678} & \ctx{1} & \ctx{1.69} & \ctx{0.82} & \ctx{\na} \\
\ctx{SoFlow-B/2~\cite{luo2026soflow}} & \ctx{\na} & \ctx{131} & \ctx{1} & \ctx{4.85} & \ctx{\na} & \ctx{\na} \\
\ctx{DMF-B/2~\cite{lee2025dmf}} & \ctx{\na} & \ctx{130} & \ctx{1} & \ctx{5.63} & \ctx{\na} & \ctx{\na} \\
\ctx{IMM-XL/2~\cite{zhou2025imm}} & \ctx{\na} & \ctx{675} & \ctx{2} & \ctx{7.77} & \ctx{\na} & \ctx{\na} \\
\ctx{Shortcut-XL/2~\cite{frans2025shortcut}} & \ctx{\na} & \ctx{676} & \ctx{1} & \ctx{10.60} & \ctx{\na} & \ctx{\na} \\
\midrule
\regrn{}-B & GRN-B & 130 & 2 & 3.73 & 1.00 & 298.6 \\
\regrn{}-L & GRN-L & 458 & 2 & 2.85 & 1.08 & 313.9 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_conf.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Refinement confidence keeping} on ImageNet $256^2$: the GRN-B teacher and the two 2-step students. Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:conf}
\footnotesize
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\grpline{6}{(a) GRN-B teacher (FID-10k)}
Sampling rule & Extra & 25 steps & Extra & 16 steps & 50 steps \\
Without keeping & 0\% & 9.59 & 0\% & 18.29 & \textbf{6.17} \\
\oursrow Refinement confidence keeping & 12\% & \textbf{6.63} & 9\% & \textbf{8.33} & \na \\
Freezing & 14\% & 8.13 & 10\% & 13.20 & \na \\
Bit keeping & 9\% & 6.67 & 5\% & 11.15 & \na \\
Bit freezing & 12\% & 10.99 & 7\% & 9.84 & \na \\
Top-confidence & \na & 146.39 & \na & \na & 91.37 \\
\grpline{6}{\quad same noise on a second L40S}
\oursrow Refinement confidence keeping & 12\% & 6.72 & 9\% & \textbf{8.35} & \na \\
Random (same share per step) & 12\% & \textbf{6.65} & 9\% & 8.67 & \na \\
Random (same total share) & 12\% & 7.00 & 9\% & 10.78 & \na \\
\midrule
\grpline{6}{(b) 2-step \regrn-B \comp{\tagW+\tagSB+\tagEH}}
Sampling rule & Extra & FID$_\mathrm{50k}$ & IS$_\mathrm{50k}$ & P$_\mathrm{T}$ & R$_\mathrm{T}$ \\
Without keeping & 0\% & 3.730 & 298.6 & 0.690 & 0.719 \\
Keeping ($a{=}0.64$) & 11\% & 3.713 & 297.9 & 0.690 & 0.718 \\
Keeping ($a{=}0.51$) & 29\% & 3.815 & 292.4 & 0.688 & 0.721 \\
Random (same share) & 11\% & 3.780 & 300.3 & 0.701 & 0.713 \\
\oursrow Trained with keeping & 29\% & 3.732 & 298.9 & 0.691 & 0.722 \\
\quad sampled without keeping & 0\% & \textbf{3.711} & 300.4 & 0.693 & 0.720 \\
\midrule
\grpline{6}{(c) 2-step \regrn-L \comp{\tagW+\tagEH}}
Sampling rule & Extra & FID$_\mathrm{50k}$ & IS$_\mathrm{50k}$ & P$_\mathrm{T}$ & R$_\mathrm{T}$ \\
Without keeping & 0\% & 3.091 & 297.2 & 0.712 & 0.709 \\
Keeping ($a{=}0.64$) & 5\% & 3.082 & 297.7 & 0.716 & 0.707 \\
Keeping ($a{=}0.51$) & 17\% & 3.107 & 294.4 & 0.712 & 0.713 \\
Random (same share) & 5\% & 3.135 & 302.3 & 0.722 & 0.703 \\
\oursrow Trained with keeping & 18\% & \textbf{3.031} & 297.7 & 0.714 & 0.716 \\
\quad sampled without keeping & 0\% & 3.084 & 299.9 & 0.714 & 0.710 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_eh_b.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Non-uniform sampling on GRN-B} (ImageNet $256^2$, 2 steps). Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:eh_b}
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}lrrrr@{}}
\toprule
\grpline{5}{(a) 2-step \tagW+\tagSB{} student (FID$_\mathrm{50k}$)}
Student (grid point $t_1$) & FID$_\mathrm{50k}$ & IS$_\mathrm{50k}$ & P$_\mathrm{T}$ & R$_\mathrm{T}$ \\
Base (\tagW+\tagSB) on $t_1{=}0.5$ & 3.826 & 306.1 & 0.712 & 0.708 \\
+2k on $t_1{=}0.5$ & 3.865 & 307.0 & 0.707 & 0.708 \\
\oursrow +2k on $t_1{=}0.25$ (NS) \comp{\tagW+\tagSB+\tagEH} & 3.730 & 298.6 & 0.690 & 0.719 \\
\quad same student sampled at $t_1{=}0.5$ & \textbf{3.637} & 297.3 & 0.704 & 0.710 \\
+2k on $t_1{=}0.33$ & 3.708 & 301.7 & 0.699 & 0.718 \\
\midrule
\grpline{5}{(b) 2-step \tagW{} student by grid point $t_1$ (FID$_\mathrm{50k}$)}
Student (grid point $t_1$) & FID$_\mathrm{50k}$ & IS$_\mathrm{50k}$ & P$_\mathrm{T}$ & R$_\mathrm{T}$ \\
Base (\tagW) on $t_1{=}0.5$ & 4.163 & 278.7 & 0.687 & 0.722 \\
+2k on $t_1{=}0.25$ & 4.378 & 264.7 & 0.673 & 0.740 \\
+2k on $t_1{=}0.33$ & 4.076 & 275.9 & 0.687 & 0.730 \\
+2k on $t_1{=}0.4$ & 4.089 & 277.6 & 0.689 & 0.726 \\
+2k on $t_1{=}0.5$ & 4.103 & 280.7 & 0.696 & 0.719 \\
+2k on $t_1{=}0.6$ & \textbf{4.036} & 286.1 & 0.699 & 0.718 \\
+2k on $t_1{=}0.67$ & 4.044 & 287.6 & 0.704 & 0.716 \\
Base sampled at $t_1{=}0.25$ & 4.634 & 269.9 & 0.664 & 0.729 \\
Base sampled at $t_1{=}0.33$ & 4.260 & 280.3 & 0.682 & 0.727 \\
Base sampled at $t_1{=}0.67$ & 4.701 & 259.1 & 0.678 & 0.721 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_eh_full.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Non-uniform sampling: full results} (ImageNet $256^2$, GRN-L, 2 steps). Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:eh_full}
\footnotesize
\setlength{\tabcolsep}{4.0pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\grpline{6}{(a) 2-step GRN-L students (FID$_\mathrm{50k}$)}
Student (grid point $t_1$) & FID$_\mathrm{50k}$ & IS$_\mathrm{50k}$ & P$_\mathrm{T}$ & R$_\mathrm{T}$ & FID-T \\
Base (10k \tagW) on $t_1{=}0.5$ & 3.648 & 310.4 & 0.7394 & 0.6610 & 2.061 \\
+2k on $t_1{=}0.5$ & 3.834 & 313.7 & 0.7459 & 0.6523 & 2.254 \\
\oursrow +2k on $t_1{=}0.25$ (NS) \comp{\tagW+\tagEH} & \textbf{3.092} & 296.4 & 0.7158 & 0.7097 & 1.594 \\
NS sampled at $t_1{=}0.5$ & 3.243 & 289.2 & 0.7142 & 0.6987 & \na \\
\midrule
\grpline{6}{(b) Grid ablations (FID-10k unless noted; $\Delta$ against the reference)}
Student (grid point $t_1$) & FID-10k & $\Delta$ & FID$_\mathrm{50k}$ & & \\
+2k on $t_1{=}0.5$ (reference) & 6.266 & 0 & 3.834 & & \\
+2k on $t_1{=}0.33$ & 5.599 & $-$0.666 & 3.136 & & \\
+2k on $t_1{=}0.25$ (NS) & 5.512 & $-$0.753 & 3.092 & & \\
+2k on $t_1{=}0.17$ & 5.780 & $-$0.486 & 3.333 & & \\
Base sampled at $t_1{=}0.25$ (untrained)$^\ast$ & 6.541 & +0.475 & 4.191 & & \\
One student for $K{=}2$ or $4$: 2 steps (\vs uniform grids 5.945) & 5.731 & $-$0.213 & & & \\
\quad 4 steps (\vs uniform grids 5.527) & 5.285 & $-$0.242 & & & \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/tab_eh_probe.tex <==
\begin{table}[t]
\centering
\caption{\textbf{What the two steps do} (ImageNet $256^2$, 2 NFE; 8 classes $\times$ 64 noises). Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:eh_probe}
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
 & & \multicolumn{2}{c}{Diversity} & Last & & \\
\cmidrule(lr){3-4}
Student & $t_1$ & draft & final & step & Kept & Chance \\
\midrule
\grpline{7}{GRN-B (\tagW)}
Base & $0.5$ & 0.110 & 0.601 & 0.596 & 0.808 & 0.251 \\
+2k on $t_1{=}0.25$ & $0.25$ & 0.155 & 0.481 & 0.809 & 0.762 & 0.288 \\
+2k on $t_1{=}0.67$ & $0.67$ & 0.118 & 0.671 & 0.449 & 0.826 & 0.253 \\
Base sampled at $t_1{=}0.25$ & $0.25$ & 0.110 & 0.398 & 0.833 & 0.669 & 0.224 \\
Base sampled at $t_1{=}0.67$ & $0.67$ & 0.110 & 0.711 & 0.420 & 0.870 & 0.262 \\
\midrule
\grpline{7}{GRN-B (\tagW+\tagSB)}
Base & $0.5$ & 0.130 & 0.588 & 0.615 & 0.770 & 0.250 \\
+2k on $t_1{=}0.25$ (NS) & $0.25$ & 0.172 & 0.484 & 0.815 & 0.739 & 0.284 \\
\midrule
\grpline{7}{GRN-L (\tagW)}
Base & $0.5$ & 0.084 & 0.500 & 0.639 & 0.721 & 0.205 \\
+2k on $t_1{=}0.25$ (NS) & $0.25$ & 0.129 & 0.413 & 0.825 & 0.698 & 0.245 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_sb_full.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Oversampling: full results} (GRN-B; FID-10k unless noted). Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:sb_full}
\footnotesize
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
 & \multicolumn{3}{c}{$N{=}2$ at iteration} & \multicolumn{2}{c}{3k} & \multicolumn{4}{c}{3k at $N{=}2$} & \multicolumn{2}{c}{3k at $N{=}2$ (50k)} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-10}\cmidrule(l){11-12}
2-step student continued with & 1k & 2k & 3k & $N{=}3$ & $N{=}4$ & P$_\mathrm{T}$ & R$_\mathrm{T}$ & FID-T & IS & FID & IS \\
\midrule
Before (10k student) \comp{\tagW} & \multicolumn{3}{c}{6.65 (start)} & 6.04 & 6.23 & 0.692 & 0.783 & 4.11 & \na & 4.17 & 277.6 \\
Original judge \comp{\tagW} & 6.50 & 6.51 & 6.50 & 6.19 & \na & 0.700 & 0.784 & 3.97 & 216.6 & 4.12 & 280.4 \\
Teacher-data judge \comp{\tagW} & 6.51 & 6.58 & 6.58 & 6.45 & \na & 0.704 & 0.783 & 3.92 & 224.3 & \na & \na \\
Oversampling judge \comp{\tagW+\tagSB} & 6.25 & 6.22 & 6.25 & 6.22 & \na & 0.705 & 0.773 & 3.92 & 233.9 & \na & \na \\
Oversampling judge (student of Tab.~\ref{tab:c2i}) \comp{\tagW+\tagSB} & 6.29 & 6.21 & 6.24 & 6.25 & 6.52 & \na & \na & \na & 234.1 & 3.83 & 306.8 \\
\bottomrule
\end{tabular}

\vspace{4pt}
\begin{tabular}{@{}lrr@{}}
\toprule
Judge fine-tuned on & CE at start & CE at 4k \\
\midrule
$R'$: own $N{=}3$ samples (2-step student) & 1.5755 & 1.5733 \\
$R_T$: teacher samples & 1.5870 & 1.5871 \\
own $N{=}8$ samples (random $K{=}3$--$6$ student) & 1.5888 & 1.5874 \\
own $N{=}5$ samples (fixed $K{=}4$ student) & 1.5843 & 1.5835 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/tab_speed.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Sampling cost per $256^2$ image.} Large-batch throughput and batch-1 latency. Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:speed}
\footnotesize
\setlength{\tabcolsep}{2.4pt}
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
 & & & \multicolumn{3}{c}{Large batch} & \multicolumn{2}{c}{Batch 1 (4090)} \\
\cmidrule(lr){4-6}\cmidrule(l){7-8}
Model & Sampler & NFE & ms/img & Net & +Dec. & ms & Gain \\
\midrule
GRN-B & Teacher & 79 & 34.9 & 1.0$\times$ & 1.0$\times$ & 835 & 1.0$\times$ \\
 & \regrn{} & 4 & 1.89 & 18.4$\times$ & 2.5$\times$ & 94 & 8.9$\times$ \\
 & \regrn{} & 2 & 0.97 & 35.8$\times$ & 2.6$\times$ & 66 & 12.7$\times$ \\
\midrule
GRN-L & Teacher & 79 & 107.3 & 1.0$\times$ & 1.0$\times$ & 1292 & 1.0$\times$ \\
 & \regrn{} & 4 & 5.62 & 19.1$\times$ & 5.3$\times$ & 111 & 11.7$\times$ \\
 & \regrn{} & 2 & 2.84 & 37.7$\times$ & 6.0$\times$ & 75 & 17.2$\times$ \\
\midrule
GRN-T2I & Teacher & 100 & 1424$^s$ & 1.0$\times$ & 1.0$\times$ & \na & \na \\
 & \regrn{} & 4 & 58.8$^s$ & 24$\times$ & 17$\times$ & \na & \na \\
 & \regrn{} & 2 & 29.1$^s$ & 49$\times$ & 27$\times$ & \na & \na \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_t2i_compare.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Few-step students of discrete text-to-image generators}, as reported. At $256^2$ unless noted; $\times$T.: GenEval relative to the method's own teacher. Notes: Sec.~\ref{sec:supp_tabnotes}.}
\label{tab:t2i_compare}
\footnotesize
\setlength{\tabcolsep}{2pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llrrrr@{}}
\toprule
Method & Teacher & Params & Steps & GenEval$\uparrow$ & $\times$T.$\uparrow$ \\
\midrule
\ctx{Di[M]O~\cite{zhu2025dimo}} & \ctx{MaskGen-L} & \ctx{0.6B} & \ctx{1} & \ctx{0.42} & \ctx{0.88} \\
\ctx{FPD~\cite{wang2026fpd}} & \ctx{MaskGen-L} & \ctx{0.6B} & \ctx{1} & \ctx{0.45} & \ctx{0.94} \\
\ctx{Soft-Di[M]O$^{g\,r}$~\cite{zhu2026softdimo}} & \ctx{MaskGen-L} & \ctx{0.6B} & \ctx{1} & \ctx{0.51} & \ctx{1.06} \\
\ctx{Soft-Di[M]O$^{g\,r\,s}$~\cite{zhu2026softdimo}} & \ctx{MaskGen-L} & \ctx{0.6B} & \ctx{1} & \ctx{0.63} & \ctx{1.31} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($256^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{2} & \ctx{0.49} & \ctx{0.84} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($256^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{4} & \ctx{0.52} & \ctx{0.88} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($512^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{2} & \ctx{0.56} & \ctx{0.83} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($512^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{4} & \ctx{0.63} & \ctx{0.93} \\
\midrule
\regrn{} & GRN-T2I & 2B & 2 & 0.67 & 0.97 \\
\regrn{} & GRN-T2I & 2B & 4 & \textbf{0.69} & \textbf{0.99} \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/tab_t2i_ctx.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Few-step text-to-image students}, GenEval overall as reported by each paper. Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:t2i_ctx}
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llrrr@{}}
\toprule
Method & Teacher & Params & Steps & GenEval$\uparrow$ \\
\midrule
\grpline{5}{Continuous}
\ctx{InstaFlow~\cite{liu2024instaflow}} & \ctx{\na} & \ctx{0.9B} & \ctx{1} & \ctx{0.33} \\
\ctx{SANA-Sprint$^g$~\cite{chen2025sanasprint}} & \ctx{\na} & \ctx{0.6B} & \ctx{1} & \ctx{0.72} \\
\ctx{SANA-Sprint$^g$~\cite{chen2025sanasprint}} & \ctx{\na} & \ctx{0.6B} & \ctx{2} & \ctx{0.76} \\
\ctx{SANA-Sprint$^g$~\cite{chen2025sanasprint}} & \ctx{\na} & \ctx{0.6B} & \ctx{4} & \ctx{0.76} \\
\ctx{SANA-Sprint$^g$~\cite{chen2025sanasprint}} & \ctx{\na} & \ctx{1.6B} & \ctx{1} & \ctx{0.76} \\
\ctx{SANA-Sprint$^g$~\cite{chen2025sanasprint}} & \ctx{\na} & \ctx{1.6B} & \ctx{2} & \ctx{0.77} \\
\ctx{SANA-Sprint$^g$~\cite{chen2025sanasprint}} & \ctx{\na} & \ctx{1.6B} & \ctx{4} & \ctx{0.77} \\
\ctx{FLUX.1-schnell$^g$~\cite{flux2024}} & \ctx{\na} & \ctx{12B} & \ctx{1} & \ctx{0.69} \\
\ctx{FLUX.1-schnell$^g$~\cite{flux2024}} & \ctx{\na} & \ctx{12B} & \ctx{2} & \ctx{0.71} \\
\ctx{FLUX.1-schnell$^g$~\cite{flux2024}} & \ctx{\na} & \ctx{12B} & \ctx{4} & \ctx{0.71} \\
\ctx{TDM~\cite{luo2025tdm}} & \ctx{\na} & \ctx{0.9B} & \ctx{4} & \ctx{0.50} \\
\ctx{LCM~\cite{luo2023lcm}} & \ctx{SDXL} & \ctx{2.6B} & \ctx{1} & \ctx{0.27} \\
\ctx{LCM~\cite{luo2023lcm}} & \ctx{SDXL} & \ctx{2.6B} & \ctx{4} & \ctx{0.51} \\
\ctx{SDXL-Turbo~\cite{sauer2024add}} & \ctx{\na} & \ctx{2.6B} & \ctx{1} & \ctx{0.55} \\
\ctx{DMD2~\cite{yin2024dmd2}} & \ctx{SDXL} & \ctx{2.6B} & \ctx{1} & \ctx{0.55} \\
\midrule
\grpline{5}{Discrete tokens}
\ctx{Di[M]O~\cite{zhu2025dimo}} & \ctx{Meissonic} & \ctx{1.0B} & \ctx{1} & \ctx{0.43} \\
\ctx{Di[M]O~\cite{zhu2025dimo}} & \ctx{MaskGen-L} & \ctx{0.6B} & \ctx{1} & \ctx{0.42} \\
\ctx{Soft-Di[M]O$^r$~\cite{zhu2026softdimo}} & \ctx{Meissonic} & \ctx{1.0B} & \ctx{1} & \ctx{0.53} \\
\ctx{Soft-Di[M]O$^{g\,r}$~\cite{zhu2026softdimo}} & \ctx{MaskGen-L} & \ctx{0.6B} & \ctx{1} & \ctx{0.51} \\
\ctx{Soft-Di[M]O$^{g\,r\,s}$~\cite{zhu2026softdimo}} & \ctx{MaskGen-L} & \ctx{0.6B} & \ctx{1} & \ctx{0.63} \\
\ctx{FPD~\cite{wang2026fpd}} & \ctx{MaskGen-L} & \ctx{0.6B} & \ctx{1} & \ctx{0.45} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($256^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{2} & \ctx{0.494} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($256^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{4} & \ctx{0.523} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($256^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{8} & \ctx{0.552} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($512^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{2} & \ctx{0.557} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($512^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{4} & \ctx{0.625} \\
\ctx{Show-o Turbo~\cite{xu2025showoturbo} ($512^2$)} & \ctx{Show-o} & \ctx{1.3B} & \ctx{8} & \ctx{0.638} \\
\midrule
\regrn{} \comp{\tagW} & GRN-T2I & 2B & 4 & \textbf{0.689} \\
\regrn{} \comp{\tagW} & GRN-T2I & 2B & 2 & 0.675 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/tab_t2i_full.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Text-to-image, GRN-T2I 2B at $256^2$: all results.} Every student is a LoRA adapter distilled from 50k teacher samples with the window (\tagW). Notes: Sec.~\ref{sec:supp_tabnotes_s}.}
\label{tab:t2i_full}
\footnotesize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{@{}lccrrrrrrrrrrrrr@{}}
\toprule
 & & & & \multicolumn{8}{c}{GenEval (553 prompts $\times$ 4 images)} & \multicolumn{4}{c}{1k COCO captions} \\
\cmidrule(lr){5-12}\cmidrule(l){13-16}
Method & $q_{\max}$ & Iter. & NFE & Overall$\uparrow$ & Single & Two & Count & Color & Pos. & Attr. & $\Delta$ vs.\ T. & FID-T$\downarrow$ & CLIP$\uparrow$ & HPS$\uparrow$ & Div.$\uparrow$ \\
\midrule
\ctx{GRN-T2I~\cite{han2026grn} ($1024^2$)$^\ast$} & \ctx{\na} & \ctx{\na} & \ctx{100} & \ctx{0.76} & \ctx{0.99} & \ctx{0.90} & \ctx{0.72} & \ctx{0.84} & \ctx{0.52} & \ctx{0.60} & \ctx{\na} & \ctx{\na} & \ctx{\na} & \ctx{\na} & \ctx{\na} \\
\midrule
Teacher (50 steps at $256^2$) & \na & \na & 100 & 0.695 & 0.98 & 0.83 & 0.71 & 0.79 & 0.33 & 0.53 & \na & 36.6$^a$ & 26.58 & 28.19 & 1.00 \\
GRN-T2I (16 steps) & \na & \na & 32 & 0.687 & 0.98 & 0.82 & 0.69 & 0.79 & 0.31 & 0.53 & $-$0.008 & 34.4 & 26.61 & 27.42 & \na \\
GRN-T2I (8 steps) & \na & \na & 16 & 0.563 & 0.93 & 0.63 & 0.52 & 0.69 & 0.24 & 0.37 & $-$0.132 & 54.5 & 26.18 & 25.07 & \na \\
GRN-T2I (4 steps) & \na & \na & 8 & 0.209 & 0.54 & 0.11 & 0.14 & 0.35 & 0.06 & 0.05 & \na & 141.3 & 22.51 & 19.41 & \na \\
GRN-T2I (2 steps) & \na & \na & 4 & 0.055 & 0.20 & 0.02 & 0.01 & 0.10 & 0.00 & 0.00 & \na & 208.4 & 17.59 & 12.44 & \na \\
Fine-tuned GRN-T2I (no CFG) & \na & \na & 50 & 0.633 & 0.94 & 0.77 & 0.60 & 0.73 & 0.29 & 0.46 & $-$0.062 & 36.5 & 26.22 & 27.11 & \na \\
Paired-noise GRN-T2I (2 steps) & \na & \na & 2 & 0.044 & 0.16 & 0.00 & 0.02 & 0.09 & 0.00 & 0.00 & \na & 209.2 & 17.95 & 15.10 & \na \\
\midrule
\regrn{} \comp{\tagW} (4 steps) & 0.40 & 2k & 4 & \textbf{0.689} & 0.99 & 0.83 & 0.68 & 0.79 & 0.29 & 0.56 & $-$0.006 & 36.0 & 26.55 & 27.28 & 0.94 \\
\regrn{} \comp{\tagW} (4 steps) & 0.55 & 1k & 4 & 0.684 & 0.99 & 0.83 & 0.66 & 0.77 & 0.30 & 0.55 & $-$0.011 & 35.6 & 26.52 & 27.32 & 0.95 \\
\regrn{} \comp{\tagW} (2 steps) & 0.40 & 4k & 2 & 0.652 & 0.96 & 0.78 & 0.66 & 0.74 & 0.27 & 0.50 & $-$0.043 & 40.3 & 26.58 & 26.50 & 0.90 \\
\regrn{} \comp{\tagW} (2 steps) & 0.55 & 2k & 2 & 0.661 & 0.97 & 0.78 & 0.67 & 0.74 & 0.31 & 0.50 & $-$0.034 & 39.1 & 26.59 & 26.58 & 0.91 \\
\regrn{} \comp{\tagW} (2 steps) & 0.55$\to$0.95 & 2k+1k & 2 & 0.675 & 0.98 & 0.80 & 0.68 & 0.78 & 0.29 & 0.52 & $-$0.020 & 36.7 & \na & \na & \na \\
\bottomrule
\end{tabular}
\end{table*}

